On the spectrum of Random Simplicial Complexes in Thermodynamic Regime

Linial-Meshulam complex is a random simplicial complex on $n$ vertices with a complete $(d-1)$-dimensional skeleton and $d$-simplices occurring independently with probability p. Linial-Meshulam complex is one of the most studied generalizations of the Erdos-Renyi random graph in higher dimensions. In this paper, we discuss the spectrum of adjacency matrices of the Linial-Meshulam complex when $np \rightarrow \lambda$. We prove the existence of a non-random limiting spectral distribution(LSD) and show that the LSD of signed and unsigned adjacency matrices of Linial-Meshulam complex are reflections of each other. We also show that the LSD is unsymmetric around zero, unbounded and under the normalization $1/\sqrt{\lambda d}$, converges to standard semicircle law as $\lambda \rightarrow \infty$. In the later part of the paper, we derive the local weak limit of the line graph of the Linial-Meshulam complex and study its consequence on the continuous part of the LSD.

==> Version 7/mypream.tex <==
%\theoremstyle{plain} %documentation says there are only three styles
                     %{plain},{definition},{remark}
    \newtheorem{theorem}{Theorem}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{claim}[theorem]{Claim}
    \newtheorem{conjecture}[theorem]{Conjecture}
%    \newtheorem{proof}[proof]{Proof}
\theoremstyle{definition} % For roman text in the body
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{fact}[theorem]{Fact}
    \newtheorem{result}[theorem]{Result}
    \newtheorem{remark}[theorem]{Remark}
    \newtheorem{example}[theorem]{Example}
    \newtheorem{exercise}[theorem]{Exercise}
    \newtheorem{algorithm}[theorem]{Algorithm}
    \newtheorem{assumption}[theorem]{Assumption}
    \newtheorem{problem}[theorem]{Problem}
    \newtheorem{notation}[theorem]{Notation}
%\newenvironment{proofof}[1]{\par \trivlist
% \itemindent\parindent \item[\hskip\labelsep\sc Proof of #1.]
% \ignorespaces}{\qed\endtrivlist}

\newtheorem{protoeg}[theorem]{Example}
\newtheorem{protoremark}[theorem]{Remark}
\newtheorem{protodefinition}[theorem]{Definition}
\renewcommand{\theequation}{\arabic{equation}}
\renewcommand{\thetheorem}{\arabic{theorem}}
%\newenvironment{theorem*}[1]{\par \trivlist
% \itemindent\parindent \item[\bf Theorem #1]
%  \it\ignorespaces}{\endtrivlist}
%\newenvironment{equation*}{$$}{$$}
%\newcommand{\qed}{\hfill\text{$\framebox(5,5)[]{}$}}
%\newcommand{\mathqed}{\framebox(5,5)[]{}}

%\renewenvironment{proof}{\par \trivlist
% \itemindent\parindent \item[\hskip\labelsep\sc Proof.]
% \ignorespaces}{\qed\endtrivlist}

\def\newblock{\hskip .11em plus .33em minus .07em}

\def\half{$\frac{1}{2}$}
\def\suchthat{\; : \;}
\def\FF{{\mathcal F}}
\def\BB{{\mathcal B}}
\def\AA{{\mathcal A}}
\def\m{\mathbf{m}}
\def\iff{\Longleftrightarrow}
\renewcommand \qedsymbol {$\blacksquare$}

%%%% end of new
%Greek letters
\def\Gam{\Gamma}
\def\Del{\Delta}
\def\Lam{\Lambda}
\def\Ome{\Omega}
\def\alp{\alpha}
\def\bet{\beta}
\def\gam{\gamma}
\def\del{\delta}
\def\eps{\epsilon}
\def\kap{\kappa}
\def\lam{\lambda}
\def\ome{\omega}
\def\Ome{\Omega}
\def\sig{\sigma}
\def\ups{\upsilon}
\def\zet{\zeta}

% Bold and mathbb fonts (to denote reals, rationals) etc
\def\II{{\mathcal I}}
\def \K{{\mathcal K}}
\def \CC{{\mathcal C}}
\def\C{\mathbb{C}}
\def\D{\mathbb{D}}
%\def\E{\mathbb{E}}
\newcommand{\E}{\mbox{E}}
\def\F{{\bf F}}
\def\G{{\bf{G}}}
\def\GG{{\mathcal G}}
%\def\H{{\bf{H}}}
\def\J{{\mathcal J}}
\def\Z{\mathbb{Z}}
\def\M{\Omega}
\def\N{\mathbb{N}}
\def\PP{{\mathcal P}}
\def\Q{{\mathbf Q}}
\def\R{\mathbb{R}}
\def\Sym{{\mathcal S}}
\def\S{\mathbb{S}}
\def\U{{\mathcal U}}
\def\X{{\mathcal X}}
\def\Y{{\mathcal Y}}
\def\Z{\mathbb{Z}}
\def\ZZ{{\mathcal Z}}
\def\ccinf{C_c^{\infty}}
\def\b{{\bf b}}
\def\c{{\bf c}}
\def\f{{\bf f}}
\def\g{{\bf g}}
\def\h{{\bf h}}
\def\a{{\bf a}}
\def\b{{\bf b}}
\def\e{{\bf e}}
\def\w{{\bf w}}
\def\m{{\bf m}}
\def\n{{\bf n}}
\def\q{{\bf q}}
\def\u{{\bf u}}
\def\v{{\bf v}}
\def\w{{\bf w}}
\def\x{{\bf x}}
\def\y{{\bf y}}
\def\z{{\bf z}}
% Some mathematical symbols, large braces etc.
\def\summ{\sum\limits}
\def\intt{\int\limits}
\def\prodd{\prod\limits}
\def\limm{\lim\limits}
\def\tends{\rightarrow}
\def\tim{\times}
\def\wed{\wedge}
\def\fr{\frac}
\def\sgn{{\mb{sgn}}}
%\newcommand{\frac}[2]{\genfrac{}{}{}{}{#1}{#2}}
%\newcommand{\tfrac}[2]{\genfrac{}{}{}{1}{#1}{#2}}
%\newcommand{\binom}[2]{\genfrac{(}{)}{0pt}{}{#1}{#2}}
%\def\sgn{\mb{sgn}}


\def\Mid{\left\vert \right.}
\def\l{\left}
\def\r{\right}
\def\<{\langle}
\def\>{\rangle}
\def\hsp{\hspace}
\def\mb{\mbox}
\newcommand{\one}{{\mathbf 1}}
\def\I#1{{\bf 1}_{#1}}
\def\per{\mb{per}}
\def\bar{\overline}
\def\P{\mbox{P}}
%\def\Var{\mbox{Var}}
\def\convd{\stackrel{d}{\rightarrow}}
\def\convp{\stackrel{P}{\rightarrow}}
\def\eqd{\stackrel{d}{=}}
\def\given{\left.\vphantom{\hbox{\Large (}}\right|}
\def\ind{{\mathbf 1}}
\def\d{\partial}
\def\dz{\frac{\partial }{ \partial z}}
\def\dzbar{\frac{\partial }{ \partial {\bar z}}}
\def\dw{\frac{\partial }{ \partial w}}
\def\dwbar{\frac{\partial }{ \partial {\bar zw}}}
\def\ccinf{C_c^{\infty}}
\def\lap{\Delta}
\def\defn{\stackrel{\tiny def}{=}}
\def\di{\mbox{d}}
\newcommand{\diff}[1]{\frac{\partial}{\partial #1}}
%\def\coin{\textrm{coin}}
%\def\sign{\textrm{sign}}


%%%%%%%%%%%%%Some common functions

\newcommand{\EE}[1]{\E\l[#1\r]}
\newcommand\Tr{{\mbox{Tr}}}
\newcommand\tr{{\mbox{tr}}}

%%%%%%%%%%%%%chapter 3 notation
\newcommand\mnote[1]{} %off
\newcommand\be{\begin{equation*}}
\newcommand\bel[1]{{\mnote{#1}}\be\label{#1}}
\newcommand\ee{\end{equation*}}
\newcommand\lb[1]{\label{#1}\mnote{#1}}
\newcommand\ben{\begin{equation}}
\newcommand\een{\end{equation}}
\newcommand\bes{\begin{eqnarray*}}
\newcommand\ees{\end{eqnarray*}}

\newcommand\bex{\begin{exercise}}
\newcommand\eex{\end{exercise}}
\newcommand\beg{\begin{example}}
\newcommand\eeg{\end{example}}
\newcommand\benu{\begin{enumerate}}
\newcommand\eenu{\end{enumerate}}
\newcommand\beit{\begin{itemize}}
\newcommand\eeit{\end{itemize}}
\newcommand\berk{\begin{remark}}
\newcommand\eerk{\end{remark}}
\newcommand\bdefn{\begin{defintion}}
\newcommand\edefn{\end{definition}}
\newcommand\bthm{\begin{theorem}}
\newcommand\ethm{\end{theorem}}
\newcommand\bprf{\begin{proof}}
\newcommand\eprf{\end{proof}}
\newcommand\blem{\begin{lemma}}
\newcommand\elem{\end{lemma}}

%
%\newcommand{\NN}{\mathcal N}
%\newcommand{\comment}[1]{}
%\newcommand{\one}{{\mathbf 1}}
\newcommand{\as}{\mbox{\hspace{.3cm} a.s.}}
\newcommand{\dist}{\mbox{\rm dist}}
\newcommand{\supp}{\mbox{\rm supp}}
\newcommand{\Arg}{\mbox{\rm Arg}}
\newcommand{\Poi}{\mbox{\rm Poi}}
\newcommand{\var}{\mbox{\rm Var}}
%\newcommand{\Tr}{\mbox{\rm Tr}}
\newcommand{\Vol}{\mbox{\rm Vol}}
\newcommand{\Cov}{\mbox{\rm Cov}}
\newcommand{\sm}{{\raise0.3ex\hbox{$\scriptstyle \setminus$}}}
\newcommand{\intc}{\int_0^{2\pi}}
\newcommand{\agau}{a complex Gaussian analytic function}
\newcommand{\gi}{\,|\,}
\newcommand{\area}{\operatorname{area}}
\newcommand{\wA}{\widetilde{A}}
\newcommand{\zb}{\overline{z}}
\newcommand{\ontop}{\genfrac{}{}{0cm}{2}}

\def\mb{\mbox}
\def\l{\left}
\def\r{\right}
\def\sig{\sigma}
\def\lam{\lambda}
\def\alp{\alpha}
\def\eps{\epsilon}
\def\tends{\rightarrow}
\def\Lap{\Delta}
%%%%%%% ST3 material
\newcommand{\const}{\operatorname{const}}

%\renewcommand{\phi}{\varphi}
\newcommand{\ip}[2]{\langle#1,#2\rangle}
\renewcommand{\Pr}[1]{\,\mathbb P\,\(\,#1\,\)\,}
\newcommand{\ti}{\tilde}
\newcommand{\Wi}[1]{:#1:}
\newcommand{\imply}{\;\;\;\Longrightarrow\;\;\;}
\def\Kdet{{\mathbb K}}

\def\STAR{\bigstar}
\def\CYCLE{\diamondsuit}
\def\CHI{\mathchoice%
{\raise2pt\hbox{$\chi$}}%
{\raise2pt\hbox{$\chi$}}%
{\raise1.3pt\hbox{$\scriptstyle\chi$}}%
{\raise0.8pt\hbox{$\scriptscriptstyle\chi$}}}
\def\smalloplus{\raise1pt\hbox{$\,\scriptstyle \oplus\;$}}
